P-FOLIO: Evaluating and Improving Logical Reasoning with Abundant Human-Written Reasoning Chains

Existing methods on understanding the capabilities of LLMs in logical reasoning rely on binary entailment classification or synthetically derived rationales, which are not sufficient for proper investigation of model's capabilities. We present P-FOLIO, a human-annotated dataset consisting of diverse and complex reasoning chains for a set of realistic logical reasoning stories also written by humans. P-FOLIO is collected with an annotation protocol that facilitates humans to annotate well-structured natural language proofs for first-order logic reasoning problems in a step-by-step manner. The number of reasoning steps in P-FOLIO span from 0 to 20. We further use P-FOLIO to evaluate and improve large-language-model (LLM) reasoning capabilities. We evaluate LLM reasoning capabilities at a fine granularity via single-step inference rule classification, with more diverse inference rules of more diverse and higher levels of complexities than previous works. Given that a single model-generated reasoning chain could take a completely different path than the human-annotated one, we sample multiple reasoning chains from a model and use pass@k metrics for evaluating the quality of model-generated reasoning chains. We show that human-written reasoning chains significantly boost the logical reasoning capabilities of LLMs via many-shot prompting and fine-tuning. Furthermore, fine-tuning Llama3-7B on P-FOLIO improves the model performance by 10% or more on three other out-of-domain logical reasoning datasets. We also conduct detailed analysis to show where most powerful LLMs fall short in reasoning. We will release the dataset and code publicly.

==> 6-models.tex <==

% \section{Improving Reasoning}
% We use abundant human-written rationales in \ours to improve LLM reasoning capabilities via fine-tuning and many-shot prompting. For fine-tuning, we evaluate under both an in-domain and an out-of-domain setting. 
% \paragraph{In-domain evaluation}
% For in-domain evaluation, we use Llama3-7B finetuned on P-FOLIO training set toe 

% \paragraph{Out-of-domain evaluation}
% For out-of-domain evaluation, we use the same fine-tuned model to evaluate on three other logical reasoning datasets, BirdElectricity, ProntoQA and bAbi-deductive. 




